A privacy-preserving tests optimization algorithm for epidemics containment

The SARS-CoV-2 outbreak changed the everyday life of almost all the people over the world.Currently, we are facing with the problem of containing the spread of the virus both using the more effective forced lockdown, which has the drawback of slowing down the economy of the involved countries, and by identifying and isolating the positive individuals, which, instead, is an hard task in general due to the lack of information. For this specific disease, the identificato of the infected is particularly challenging since there exists cathegories, namely the asymptomatics, who are positive and potentially contagious, but do not show any of the symptoms of SARS-CoV-2. Until the developement and distribution of a vaccine is not yet ready, we need to design ways of selecting those individuals which are most likely infected, given the limited amount of tests which are available each day. In this paper, we make use of available data collected by the so called contact tracing apps to develop an algorithm, namely PPTO, that identifies those individuals that are most likely positive and, therefore, should be tested. While in the past these analysis have been conducted by centralized algorithms, requiring that all the app users data are gathered in a single database, our protocol is able to work on a device level, by exploiting the communication of anonymized information to other devices.

==> basic_evolution.tex <==
% This file was created by tikzplotlib v0.8.2.
\begin{document}

\begin{tikzpicture}

\definecolor{color0}{rgb}{0.917647058823529,0.917647058823529,0.949019607843137}
\definecolor{color1}{rgb}{0.298039215686275,0.447058823529412,0.690196078431373}
\definecolor{color4}{rgb}{0.768627450980392,0.305882352941176,0.32156862745098}
\definecolor{color2}{rgb}{0.866666666666667,0.517647058823529,0.32156862745098}
\definecolor{color3}{rgb}{0.333333333333333,0.658823529411765,0.407843137254902}

\begin{axis}[
axis background/.style={fill=color0},
axis line style={white},
legend cell align={left},
legend style={at={(0.03,0.97)}, anchor=north west, draw=white!80.0!black, fill=color0},
tick align=outside,
tick pos=both,
x grid style={white},
xmajorgrids,
xmin=-1.45, xmax=30.45,
xtick style={color=darkgray!60.0!black},
y grid style={white},
ymajorgrids,
ymin=-134.3, ymax=2820.3,
ytick style={color=darkgray!60.0!black}
]
\addplot [semithick, color1, dashed]
table {%
0 1
1 4
2 9
3 12
4 19
5 29
6 38
7 57
8 74
9 94
10 114
11 131
12 162
13 195
14 238
15 283
16 349
17 433
18 533
19 620
20 771
21 920
22 1104
23 1296
24 1475
25 1704
26 1956
27 2235
28 2467
29 2686
};

\addplot [semithick, color2, dashed]
table {%
0 0
1 0
2 0
3 0
4 0
5 0
6 3
7 3
8 5
9 6
10 11
11 12
12 18
13 23
14 27
15 30
16 32
17 38
18 38
19 42
20 55
21 75
22 95
23 107
24 123
25 138
26 149
27 169
28 184
29 211
};

\addplot [semithick, color3, dashed]
table {%
0 5
1 5
2 5
3 5
4 5
5 4
6 4
7 4
8 3
9 4
10 3
11 4
12 5
13 6
14 7
15 8
16 11
17 16
18 27
19 31
20 37
21 42
22 47
23 58
24 65
25 79
26 97
27 114
28 139
29 155
};

\addplot [semithick, color4, dashed]
table {%
0 0
1 0
2 0
3 0
4 0
5 1
6 1
7 1
8 2
9 2
10 3
11 3
12 3
13 3
14 3
15 3
16 3
17 4
18 4
19 4
20 4
21 5
22 6
23 6
24 10
25 11
26 13
27 17
28 19
29 25
};

\end{axis}

\end{tikzpicture}
\end{document}

